S-Isomap++: Multi Manifold Learning from Streaming Data

Manifold learning based methods have been widely used for non-linear dimensionality reduction (NLDR). However, in many practical settings, the need to process streaming data is a challenge for such methods, owing to the high computational complexity involved. Moreover, most methods operate under the assumption that the input data is sampled from a single manifold, embedded in a high dimensional space. We propose a method for streaming NLDR when the observed data is either sampled from multiple manifolds or irregularly sampled from a single manifold. We show that existing NLDR methods, such as Isomap, fail in such situations, primarily because they rely on smoothness and continuity of the underlying manifold, which is violated in the scenarios explored in this paper. However, the proposed algorithm is able to learn effectively in presence of multiple, and potentially intersecting, manifolds, while allowing for the input data to arrive as a massive stream.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> motivation.tex <==
Our motivation for this work stems from one of the foundation principles of {\em Manifold Learning}, which assumes that the distribution of the data in the high-dimensional observed space is not uniform and in reality, the data lies near a non-linear low-dimensional manifold embedded in the high-dimensional space. In many real-world problems such as those resulting from multi-modal or unevenly sampled distributions, the data lies on multiple manifolds of possibly different ``dimensionalities'' and is typically separated by regions of low density as depicted in Figure~\ref{fig:mnist_data}. Thus, to find a representative low-dimensional embedding of the data, one needs to first cluster the data appropriately and subsequently find a low-dimensional representation for the data in each cluster. Even then, manifolds can be very close to each other and can have arbitrary intrinsic dimensions, curvature and sampling which makes it a hard problem to solve.

In the ideal scenario, when manifolds are densely sampled and sufficiently separated, existing NLDR methods can be extended to perform clustering before applying the dimensionality reduction step~\cite{polito2002, goh2008,fan2012}, by choosing an appropriate local neighborhood size so as not to include points from other manifolds and still be able to capture the local geometry of the manifold. 

The Isomap algorithm, being a global NLDR technique should ideally provide a more faithful representation and preserve geometry irrespective of scale i.e. map data samples are close in the manifold to points which are close in the low-dimensional embedding and similarly for distant samples, however, it struggles when dealing with multi-modal and non-uniform distributions.

NLDR techniques, irrespective of whether they are global or local, require an appropriate choice of the neighborhood size ($k$) to define their local neighborhood to perform appropriately. More specifically, a small neighborhood size might not to capture sufficient information about the manifold geometry, more so when it is smaller than the intrinsic dimensionality of the manifold. A large neighborhood size could lead to issues i.e. short-circuiting when distant, far-off get included in the local neighborhood and corrupt the same. Idiosyncrasies i.e. curvature and uneven sampling in different regions of the manifold make choosing the problem of choosing the local neighborhood size particularly difficult. The Isomap algorithm is also not immune to the above. When the sampling or distribution of data is multi-modal and non-uniform, we are forced to choose a large $k$ value so that we can formulate the Geodesic distance matrix for all the data points, which would enable the Isomap algorithm to perform dimensionality reduction. In such scenarios, short-circuiting results in improper embeddings uncovered by Isomap, which typically needs smaller values of $k$ to appropriately represent the local neighborhood. 

This particular issue can be seen in Figure~\ref{fig:patches} where both the M-Isomap~\cite{fan2012} and S-Isomap++ algorithms can deal with individual manifolds well compared to Isomap which severely deforms the individual clusters, which are $\mathbb{R}^2$ Gaussian distributions mapped to $\mathbb{R}^3$ via the Isometric technique suggested by Schoeneman \emph{et al.}~\cite{schoeneman2017}. It should also be noted that whereas both the M-Isomap and S-Isomap++ algorithms required small values of $k$ i.e. $k=8$ to operate, Isomap needed values of $k \geq 500$ to even work. 

